A Systematic Comparison of Contextualized Word Embeddings for Lexical Semantic Change

Contextualized embeddings are the preferred tool for modeling Lexical Semantic Change (LSC). Current evaluations typically focus on a specific task known as Graded Change Detection (GCD). However, performance comparison across work are often misleading due to their reliance on diverse settings. In this paper, we evaluate state-of-the-art models and approaches for GCD under equal conditions. We further break the LSC problem into Word-in-Context (WiC) and Word Sense Induction (WSI) tasks, and compare models across these different levels. Our evaluation is performed across different languages on eight available benchmarks for LSC, and shows that (i) APD outperforms other approaches for GCD; (ii) XL-LEXEME outperforms other contextualized models for WiC, WSI, and GCD, while being comparable to GPT-4; (iii) there is a clear need for improving the modeling of word meanings, as well as focus on how, when, and why these meanings change, rather than solely focusing on the extent of semantic change.

==> Ninas-version.tex <==
\section{Introduction}
Lexical Semantic Change (LSC) is the task of computationally identifying words that change their meaning over time~\cite{montanelli2023survey,tahmasebi2018survey,kutuzov2018diachronic}. The interest in this task has been significantly fueled by the advent of word embeddings and modern language models. %in Natural Language Processing (NLP), 
After years of ad hoc evaluation, a new evaluation framework was introduced, aimed at assessing and comparing the accuracy of different computational approaches~\cite{schlechtweg2020semeval}. The framework was proposed as shared task where participants were provided of a diachronic corpus spanning two time periods, along with a list of target words. The challenge encompassed two subtasks: i) \textbf{Binary Change Detection}: classify each target word as having gained or lost senses between the time period, and ii) \textbf{Graded Change Detection}: rank the targets based on their degree of semantic change. 

Notably, these tasks differ significantly, as words demonstrating a high degree of semantic change may not necessarily have gained or lost senses over time. Instead, one sense can have increased in prevalence, or an existing sense can taken over the role as the dominant sense. Conversely, words with a low degree of overall change may have undergone subtle shifts in their senses, e.g. by adding a low-frequent sense (see Figure~\ref{fig:semeval-de} for a relation between graded and binary change in the German data). 

While the graded sense change task was developed to measure complementary change to the binary one, it has received a disproportionate focus because of the current methods used to tackle LSC. %Francesco: I have different opinions on the entire paragraph
When the evaluation framework and the shared task was launched, methods building on static embeddings were dominant. Because static embeddings offer only one representation per word, they are incapable of differentiating between senses and thus less suitable to solve the binary task.
Contextual models, which have since dominated the LSC models, provide a representation for each instance of a word, i.e., type vectors. Potentially, these could be grouped to capture meaning distinctions, i.e., senses and could thus offer better solutions for binary change. However, most often, no such grouping is made. Instead, all vectors are used to capture signals of change, much like the static one-vector-per-word paradigm. 

The graded task remains the basis and the binary (sense gain and loss) task is seen as a binarization of the graded task: words with sufficiently high graded change have also experienced sense gain or loss. However, such a view is insufficient when deeper studies of individual words are needed, in particular on the level of individual senses. The graded change, that captures a signal of change, can however  add information when the set of senses are not changed, but the senses themselves are changed. It can also serve as a brute measure of semantic change on the level of the vocabulary, e.g., to quantify periods or genres in which much change has occurred. 

In this paper, we will make two main contributions: 
Prompted by the scalability challenges posed by handling a substantial number of contextualized embeddings, both in terms of time and space, researchers and practitioners have evaluated their approaches in diverse settings, making it challenging to compare performance in a fair and consistent manner.
Therefore, our first contribution is a \textbf{systematic evaluation} of various models and approaches for Graded Change Detection under the same conditions. 
Secondly, we will provide a discussion on \textbf{future modeling paradigms} for LSC and the highlight the importance of going beyond the graded change detection task. 


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{img/semeval-de.png}
    \caption{Gold binary labels and continuous scores for the Graded and Binary Change Detection tasks in the German benchmark~\cite{schlechtweg2020semeval}.}
    \label{fig:semeval-de}
\end{figure}



%Related Work??
%LSC was set in realistic unsupervised scenarios across four languages, i.e.~English (EN), German (DE), Swedish (SW), and Latin (LA), with benchmarks that encompassed test sets without train and dev sets. Following the success of SemEval-2020, new shared tasks were organized for additional languages, including Spanish (SP)~\cite{zamora2022lscdiscovery}, Italian (IT)~\cite{basile2020diacr}, and Russian (RU)~\cite{kutuzov2021rushifteval}, while benchmarks for languages such as Norwegian (NO) and Chinese (ZH) were also introduced~\cite{kutuzov2022nordiachange,chen2022lexicon}.

%The initial excitement for word embeddings prompted researchers and practitioners to model semantic change through static embedding models such as Word2Vec. However, the shift towards more advanced Transformer architectures has established the use of contextualized embeddings as preferred tool for addressing LSC. 




%While the initial enthusiasm for word embeddings have led researchers and practitioners to model semantic change using static embedding models like Word2Vec~\cite{tahmasebi2018survey,kutuzov2018diachronic}, the adoption of dynamically contextualized embedding models has shown superior performance in shared competitions. Consequently, these models have emerged as the preferred tools for addressing LSC tasks~\cite{montanelli2023survey}. However, the introduction of larger and contextualized models has presented a scalability challenge in handling various aspects of model training, fine-tuning, and embedding generation. Notably, these models generate vector representations per word occurrence (token embedding) rather than per word (word embedding). This, combined with the unsupervised scenario lacking a training set, gives rise to two significant issues. Firstly, the Graded Change Detection task has received more attention, as it does not require threshold tuning and can be addressed by simply computing the similarity between vectors. Conversely, the Binary Change Detection task has been relatively overlooked. Secondly, researchers and practitioners have evaluated their approaches in somewhat different settings. For example, some work utilized the full diachronic corpora to estimate the change of each target, while others used only a small sample of the full corpora (e.g., ranging from 50 to 250 uses per target word). Additionally, some work relied solely on the original annotated samples, from which both the gold labels for Binary Change Detection and the gold scores for Grade Change Detection were derived. Although it is commonly assumed that LSC results are comparable, there are risks of potential inaccuracies in semantic shift evaluation~\cite{liu2021statistically}. Word embeddings have demonstrated varying stability across term frequencies~\cite{zhou2022problems,Leszczynski2020Understanding}, and most of the available benchmark provide a small test set (e.g.~37 target words for English), which often consists of skewed distribution of change scores~\cite{kutuzov2020uio}. Consequently, the evaluation of computational methods for Graded Change Detection may be particularly biased to these issues. 

%Addressing Graded Change Detection warrants a critical examination of its utility, especially considering its distinction from Binary Change Detection. In this context, words that remain unchanged over time may exhibit a high degree of change in Graded Change Detection, indicative of a different form of change involving the acquisition or loss of meanings. Conversely, Binary Change Detection may associate a low degree of change with words that have undergone semantic shifts. This disparity prompts a fundamental question regarding the task's value for historical linguistics research. If the computational methods developed for this task fail to provide a nuanced interpretation of semantic change, the relevance of Graded Change Detection within the broader context of historical linguistics becomes questionable.


\section{Related work}
We recently proposed a comprehensive classification framework for CSSDetection~\citep{periti2023survey}, which distinguishes approaches based on three dimensions of analysis: \textit{meaning representation, time-awareness, and learning modality}. 

Meaning representation concerns the representation of word meanings: i) \textit{form-based} approaches focus on high-level properties of
a word, such as its dominant meaning or its degree of polysemy; on the opposite ii) \textit{sense-based} approaches focus on low-level properties of a word, i.e. its multiple and different meanings. 

Time-awareness focuses on how the time information of the documents is considered in the embedding model: i) \textit{time-oblivious} approaches do not consider the time at which a document is inserted in the corpus; on the opposite ii) \textit{time-aware} approaches use a specific mechanism to encode the time information into the embeddings. 

Learning modality is about the possible use of external knowledge for describing and learning the word meanings or the semantic shift to recognise: i) \textit{supervised} approaches exploit external knowledge such as a dictionary or human-annotated dataset; on the opposite ii) \textit{unsupervised} approaches derive word meanings/semantic shift from the text in the corpus by using unsupervised learning techniques. 

\subsection{Approaches to CSSDetection}
Usually, CSSDetection approaches follow a three-step scheme: i) extraction of embeddings for each occurrence of a target word from a contextualised language model such as BERT, ELMo, or XLM-R; ii) an optional aggregation of the embeddings by averaging and/or clustering; and iii) the application of a semantic shift function like Cosine Distance or Jensen-Shannon Divergence. 

For the sake of clarity, in the following, we present the main solutions according to the meaning representation of the considered target word, namely form- and sense- based approaches, respectively.

\paragraph{Form-based approaches.}
Word embeddings are optionally aggregated by averaging in a single representation, and used as input of a semantic shift function. On the one hand, form-based approaches that aggregate embeddings tend to detect the shift of the dominant meaning of the word $w$ (e.g., \citep{martinc2020leveraging}). On the other hand, form-based approaches that do not aggregate embeddings tend to detect the shift in the degree of the polysemy of the word (e.g., \citep{giulianelli2020analysing}). 

Most form-based approaches follow the general scheme and are time-oblivious. A few time-aware approaches have been recently published and they are all characterised by the adoption of a specific fine-tuning operation to inject time information into the embedding model before assessing the semantic shift of a word (e.g., \citep{hofmann2021dynamic}). 

All existing form-based approaches leverage unsupervised learning modalities. As an exception, a Word-in-Context model (WiC) is trained in \citep{arefyev2021deep} to reproduce the behavior of human annotators in the manual annotation task.

\paragraph{Sense-based approaches.}
In sense-based approaches, word embeddings are usually aggregated by clustering (e.g., \citep{giulianelli2020analysing}). All the documents of two time periods are considered as a whole, and a single clustering activity is performed, generating clusters with documents of different time periods. The idea is that each cluster denotes a specific word meaning that can be recognised in the considered documents. In this way, it is possible to assess and quantify the shift in meaning of a word by analysing the cluster membership of the documents.  

All existing sense-based approaches are time-oblivious and most leverage unsupervised learning modalities. A number of unsupervised clustering algorithms (e.g., K-Means~\citep{giulianelli2020analysing}) are proposed to sidestep the need of lexicographic resources. %Then, a general shift assessment of a word is measured by exploiting a shift function over the cluster membership of the two considered time periods (e.g., JSD~\citep{martinc2020capturing}).

Only a few approaches employ a lexicographic supervision. For instance, a supervised clustering is enforced in \citep{hu2019diachronic} by leveraging a reference dictionary (i.e., the Oxford English dictionary) to list the possible lexicographic meaning of a word beforehand; thus it is hardly
applicable to low-resource languages.  

Contrary to form-based approaches, sense-based approaches enable the semantic shift interpretation by performing an in-depth qualitative analysis of the resulting clusters. For instance, a cluster is often inspected by selecting the documents associated with the top closest vectors to its cluster centroid (e.g.,~\citep{giulianelli2020analysing}) or its most discriminating Tf-Idf keywords (e.g.,~\citep{montariol2021scalable}). However, when more than two time periods are considered, clusters of word meanings need to be re-calculated, meaning that scalability issues arise and that resulting clusters could dramatically change from one time period to the next. Thus, the possible evolution patterns of a meaning across different time periods cannot be captured. As a possible solution, some recent works propose to perform clustering separately for each time period. In this case, the resulting clusters need to be aligned in order to recognise similar word meanings in different, consecutive time periods (e.g.,~\citep{montariol2021scalable}). To avoid continuously re-calculating and aligning clusters, we propose to use an incremental clustering algorithm to trace the evolution of clusters/word meanings over time~\citep{periti2022what}.

\subsection{Graded Change Detection}

\subsection{Classification framework}

\section{Methodology}

To ensure a rigorous and systematic comparison among state-of-the-art (SOTA) approaches, we carefully selected four widely adopted and powerful form-based and sense-based methods. Each approach underwent evaluation under diverse conditions, as outlined in the classification framework proposed by Montanelli and Periti. These conditions included variations in languages, benchmarks, and embeddings derived from distinct models and layers.

For the sake of simplicity, we chose to assess the performance of different approaches using pre-trained models, aligning with the unsupervised nature of SemEval.

\subsection{Benchmarks}

Our comparative analysis leveraged all available benchmarks for the Graded Change Detection task, spanning various languages, time periods, and test set sizes. These benchmarks adhere to the novel annotation paradigm for word senses known as Word Usage Graphs (WUGs) (Schlechtweg et al., 2020, 2021b).

In this paradigm, human annotators provide semantic proximity judgments for pairs of word usages (Word-in-Context). These judgments are then encapsulated in a weighted graph and subjected to clustering via a graph clustering algorithm, as illustrated in Figure 1. Word sense clusters are consequently inferred from simple pairwise word usage judgments, obviating the need for explicit word sense definitions. The ground truth for lexical semantic change, represented as a continuous score of change, is computed for each target word by comparing the cluster distributions of time-specific usages.

Details for each benchmark, including the current state-of-the-art performance for reference purposes, are presented in Table 1. A set of available benchmarks contains both the derived graded scores per target word and the raw judgments provided by annotators for every annotated pair. To ensure the most controlled experiment, we decided to compare approaches in detecting changes in the sentences used for building the graph instead of using the full corpora from which sentences were extracted. This means that our corpora C1 and C2 are represented by all and only the sentences from C1 and from C2 annotated.

\subsection{Contextualized Word Embeddings}

In our comparison, we included the most commonly used contextualized models, both monolingual and multilingual, such as BERT, mBERT, and XLM-R for each benchmark. Additionally, we incorporated a novel model that has recently achieved state-of-the-art performance in English, Swedish, Latin, and [mention the additional language]. Our pipeline is consistent for every model. Given a word, we collect contextualized word embeddings by individually feeding the models with each sentence in which the word occurs (i.e., word usage). We then extract contextualized embeddings generated at the top (i.e., last layer) of the model for the word in the input context. We rely on the contextualized nature of these representations for detecting and ranking signals of meaning change.

\subsection{Measuring Semantic Change}
APD
PRT
AP
WiDiD

\subsection{Experimental results}
\subsection{Form-based vs Sense-based}
\subsection{Time-oblivious vs Time-aware}



\begin{table*}[!ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccc}
 &  &  & \textbf{EN} & \textbf{LA} & \textbf{DE} & \textbf{SV} & \textbf{ES} & \multicolumn{3}{c}{\textbf{RU}} & \multicolumn{2}{c}{\textbf{NO}} & \textbf{ZH} \\ \cline{4-14} 
 &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textit{$C_1 - C_2$}} & \multicolumn{1}{c|}{\textit{$C_1 - C_2$}} & \multicolumn{1}{c|}{\textit{$C_1 - C_2$}} & \multicolumn{1}{c|}{\textit{$C_1 - C_2$}} & \multicolumn{1}{c|}{\textit{$C_1 - C_2$}} & \textit{$C_1 - C_2$} & \textit{$C_2 - C_3$} & \multicolumn{1}{c|}{\textit{$C_1 - C_3$}} & \textit{$C_1 - C_2$} & \multicolumn{1}{c|}{\textit{$C_2 - C_3$}} & \multicolumn{1}{c|}{\textit{$C_1 - C_2$}} \\ \cline{2-14} 
\multicolumn{1}{l|}{\multirow{2}{*}{\rotatebox{90}{\textbf{form-based}}}} & \multicolumn{1}{c|}{APD} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BERT\\ mBERT\\ XLM-R\\ XLL\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.563\\ .363\\ .444\\ \textbf{.886}*\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-\\ .102\\ .151\\ \textbf{.231}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.271\\ .398\\ .264\\ \textbf{.839}*\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.270\\ .389\\ .257\\ \textbf{.812}*\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.336\\ .401\\ .342\\ \textbf{.560}*\end{tabular}} & \begin{tabular}[c]{@{}c@{}}.518\\ .368\\ .290\\ \textbf{.796}*\end{tabular} & \begin{tabular}[c]{@{}c@{}}.482\\ .345\\ .287\\ \textbf{.820}*\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.416\\ .386\\ .318\\ \textbf{.863}*\end{tabular}} & \begin{tabular}[c]{@{}c@{}}.441\\ .279\\ .195\\ \textbf{.659}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.466\\ .488\\ .379\\ \textbf{.640}*\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.656\\ .689\\ .500\\ \textbf{.731}*\end{tabular}} \\ \cline{2-14} 
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{PRT} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BERT\\ mBERT\\ XLM-R\\ XLL\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.457\\ .270\\ .411\\ \textbf{.676}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-\\ .380\\ .424\\ \textbf{.506}*\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.422\\ .436\\ .369\\ \textbf{.824}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.158\\ .193\\ .020\\ \textbf{.696}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.392\\ \textbf{.539}\\ .453\\ .494\end{tabular}} & \begin{tabular}[c]{@{}c@{}}.400\\ .391\\ .321\\ \textbf{.704}\end{tabular} & \begin{tabular}[c]{@{}c@{}}.374\\ .356\\ .443\\ \textbf{.750}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.347\\ .423\\ .405\\ \textbf{.727}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}.507\\ .219\\ .387\\ \textbf{.764}*\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.444\\ .438\\ .149\\ \textbf{.519}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{.712}\\ .524\\ .558\\ .699\end{tabular}} \\ \cline{2-14} 
\multicolumn{1}{l|}{\multirow{2}{*}{\rotatebox{90}{\textbf{sense-based}}}} & \multicolumn{1}{c|}{AP} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BERT\\ mBERT\\ XLM-R\\ XLL\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.289\\ .181\\ .278\\ \textbf{.493}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-\\ .277\\ \textbf{.398}\\ .033\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.469\\ .280\\ .224\\ \textbf{.499}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}- .090\\ .023\\  -.076\\ \textbf{.118}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.210\\ .101\\ .126\\ \textbf{.278}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}.069\\ .017\\ - .068\\ \textbf{.106}\end{tabular} & \begin{tabular}[c]{@{}c@{}}.279\\ .086\\ \textbf{.209}\\ .053\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.094\\ - .116\\ \textbf{.130}\\ .117\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\textbf{.314}\\ .035\\ - .100\\ .297\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.011\\ - .090\\ .030\\ \textbf{.381}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.165\\ .465\\ .448\\ \textbf{.308}\end{tabular}} \\ \cline{2-14} 
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{WiDiD} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BERT\\ mBERT\\ XLM-R\\ XLL\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.385\\ .323\\ .564\\ \textbf{.652}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-\\ - .0.39\\ - .064\\ \textbf{.236}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.355\\ .312\\ .499\\ \textbf{.677}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.106\\ .195\\ .129\\ \textbf{.475}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.251\\ .417\\ .390\\ \textbf{.417}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}.135\\ - .068\\ \textbf{.268}\\ .178\end{tabular} & \begin{tabular}[c]{@{}c@{}}.102\\ .160\\ .216\\ \textbf{.354}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.243\\ .142\\ .342\\ \textbf{.364}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}.233\\ .241\\ .226\\ \textbf{.561}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.087\\ .290\\ .349\\ \textbf{.457}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.533\\ .338\\ .382\\ \textbf{.563}\end{tabular}} \\ \cline{2-14} 
\end{tabular}%
}
\caption{Todo}
\label{tab:form-vs-sense}
\end{table*}
\cite{pilehvar2019wic}

%notes: è normale hce i modelli form siano più avantaggiati poichè mancano di uno step intermedio

Why? -> Word-in-Context
Word Sense Induction
Semantic Change

\subsection{Other dimension of comparison}
\paragraph{Layers}
\paragraph{Layers aggregation}
\paragraph{Monolingual vs Multilingual}
\paragraph{Semantic change measures}
Are models time-awarness? Can model contextualize?
are cosine best for LSC?
are the last four layers the best for addressing LSC?
are monolingual model better for addressing LSC?

\section{Time-aware vs. Time-oblivious: Should we model time-aware model?}
The consideration of time awareness in embedding models focuses on how temporal information is integrated into the model when processing documents. Time-oblivious approaches operate under the assumption that a document at time t inherently adopts linguistic patterns reflective of the language at the same time, rendering unnecessary the explicit incorporation of time information into the embedding model. In contrast, time-aware approaches assume that contextualized embedding models face challenges in adapting to temporal shifts and generalizing over time, as they are typically pre-trained on corpora derived from a snapshot of the web collected at a specific moment. Given that our model demonstrates transfer learning capabilities across languages, we posit that the model can adapt to temporal changes within the same languages as most of significant portion of words maintains stability over time\cite{}. Despite the contextualization potential of models, especially in cross-linguistic scenarios, caution is warranted when working with a small language unit, such as word occurrences. Even though contextualized models can adapt to linguistic changes, they fall short when it comes to contextualizing word meanings beyond their training scope. This limitation is demonstrated through simple experiments emulating semantic change, detailed in our forthcoming paper X [currently under review].

This limitation underscores the advantages of form-based approaches in Grand Change Detection. Given the model's inability to contextualize word meanings beyond their training data, clustering algorithms struggle to disambiguate meanings for which the model lacks training. In contrast, form-based approaches can leverage embeddings that are more spatially distant to effectively model semantic changes.



\section{Supervised vs Unsupervised: is supervision the way?}
Approaches leveraging a form of supervision have demonstrated significantly greater efficacy for Lexical Semantic Change (LSC) than unsupervised models. We posit that supervision should be embraced to enhance the contextualization capabilities of the model or its awareness of the underlying meaning it was trained upon, rather than merely augmenting its 'pre-trained' knowledge of word meanings. This is particularly crucial given the dynamic nature of language or few-resources languages; meanings that diverge from the injected pre-trained knowledge may be inadequately represented, echoing the challenges faced by unsupervised models of semantic change.

While it is undeniable that models like GPT showcase exceptional proficiency in generating sense definitions, representing the forefront of AI with continuous updates, their strength lies in modeling present and future definitions. However, they might falter when tasked with producing definitions for the past, as exemplified in Table X. Therefore, we contend that fine-tuning may offer a more adaptable approach, even in the absence of explicit supervision.



\section{XL-Lexeme vs ChatGPT per LSC}

\section{Towards a new generation LSC}
massive graded change ha senso solo over time petr torvare il punto di cambiamento
binary change is not reliable dobbiamo rimodellarlo
dobbiamo modellare binary e sense -> 


\section{Related work}

\section{Conclusion}










==> tmp.tex <==
\section{Introduction}
Lexical Semantic Change (LSC) is the task of automatically identifying words that change their meaning over time~\cite{montanelli2023survey,tahmasebi2018survey,kutuzov2018diachronic}. The interest in this task has been significantly fueled in Natural Language Processing (NLP) by the advent of word embeddings and modern language models, leading to the development of a new evaluation framework aimed at assessing and comparing the accuracy of different computational approaches~\cite{schlechtweg2020semeval}.  %Nina: Here i would turn the order a bit, it is not that LSC was set in a realistic scenario that lead to the disproportionate focus on graded change... I will soon writ emore: Yes, you may be right, but I think a changed focus could still make it easier to get the main point through. 
%Also, I think in this paper /intro, you can think in the same way as for the proposal writing. Write your "in a nutshell" 3-5 sentence summary first, what are your main points. Perhaps we have different main points :)

% Francesco: ok, I will do it, by the way.. i thought the intro was almoast finished, than i start thinking we have different perspectives
% you are free to change it, I am now working a bit on the followings in order to make my thoughts clearer to you, than change as you prefer

% Ok! I also don't propose very large changes, just slight shifts in focus and perhaps a bit more of a discussion on what exactly graded change could capture, and in contrast, what it is being used for now. so a problematization of graded change. But , I will read the intro a few times and then make changes and let you know when I'm done. 

%ok. my big issue is frame the comparison in table 1. I will be ok for every flow.

%ok. I'll let you know

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{img/semeval-de.png}
    \caption{Gold binary labels and continuous scores for the Graded and Binary Change Detection tasks in the German benchmark~\cite{schlechtweg2020semeval}.}
    \label{fig:semeval-de}
\end{figure}

Prompted by the scalability challenges posed by handling a substantial number of contextualized embeddings, both in terms of time and space, researchers and practitioners have evaluated their approaches in diverse settings, making it challenging to compare performance in a fair and consistent manner. For instance, some studies utilized the entire diachronic corpus to estimate the change of each target, while others relied on smaller samples (e.g., ranging from 30 to 250 word usages per target word). Since most available benchmarks comprise a limited test set (e.g., 40 target words), often characterized by a skewed distribution of change scores~\cite{kutuzov2020uio}, the evaluation and comparison of computational methods for Graded Change Detection may be particularly prone to be biased. This is especially true as recent work has shown that semantic change may be either inflated or underestimated due to the varying stability of embeddings influenced by word frequencies~\cite{liu2021statistically, martinc2020capturing}.

In this paper, motivated by the remarkable performance of a recently published model for LSC~\cite{cassotti2023xl}, we conducted a systematic evaluation of various models and approaches for Graded Change Detection. Our investigation aligns with the dimensions of analysis emphasized in a recent survey~\cite{montanelli2023survey}, providing insights into the current status of LSC in NLP.



%Related Work??
%LSC was set in realistic unsupervised scenarios across four languages, i.e.~English (EN), German (DE), Swedish (SW), and Latin (LA), with benchmarks that encompassed test sets without train and dev sets. Following the success of SemEval-2020, new shared tasks were organized for additional languages, including Spanish (SP)~\cite{zamora2022lscdiscovery}, Italian (IT)~\cite{basile2020diacr}, and Russian (RU)~\cite{kutuzov2021rushifteval}, while benchmarks for languages such as Norwegian (NO) and Chinese (ZH) were also introduced~\cite{kutuzov2022nordiachange,chen2022lexicon}.

%The initial excitement for word embeddings prompted researchers and practitioners to model semantic change through static embedding models such as Word2Vec. However, the shift towards more advanced Transformer architectures has established the use of contextualized embeddings as preferred tool for addressing LSC. 




%While the initial enthusiasm for word embeddings have led researchers and practitioners to model semantic change using static embedding models like Word2Vec~\cite{tahmasebi2018survey,kutuzov2018diachronic}, the adoption of dynamically contextualized embedding models has shown superior performance in shared competitions. Consequently, these models have emerged as the preferred tools for addressing LSC tasks~\cite{montanelli2023survey}. However, the introduction of larger and contextualized models has presented a scalability challenge in handling various aspects of model training, fine-tuning, and embedding generation. Notably, these models generate vector representations per word occurrence (token embedding) rather than per word (word embedding). This, combined with the unsupervised scenario lacking a training set, gives rise to two significant issues. Firstly, the Graded Change Detection task has received more attention, as it does not require threshold tuning and can be addressed by simply computing the similarity between vectors. Conversely, the Binary Change Detection task has been relatively overlooked. Secondly, researchers and practitioners have evaluated their approaches in somewhat different settings. For example, some work utilized the full diachronic corpora to estimate the change of each target, while others used only a small sample of the full corpora (e.g., ranging from 50 to 250 uses per target word). Additionally, some work relied solely on the original annotated samples, from which both the gold labels for Binary Change Detection and the gold scores for Grade Change Detection were derived. Although it is commonly assumed that LSC results are comparable, there are risks of potential inaccuracies in semantic shift evaluation~\cite{liu2021statistically}. Word embeddings have demonstrated varying stability across term frequencies~\cite{zhou2022problems,Leszczynski2020Understanding}, and most of the available benchmark provide a small test set (e.g.~37 target words for English), which often consists of skewed distribution of change scores~\cite{kutuzov2020uio}. Consequently, the evaluation of computational methods for Graded Change Detection may be particularly biased to these issues. 

%Addressing Graded Change Detection warrants a critical examination of its utility, especially considering its distinction from Binary Change Detection. In this context, words that remain unchanged over time may exhibit a high degree of change in Graded Change Detection, indicative of a different form of change involving the acquisition or loss of meanings. Conversely, Binary Change Detection may associate a low degree of change with words that have undergone semantic shifts. This disparity prompts a fundamental question regarding the task's value for historical linguistics research. If the computational methods developed for this task fail to provide a nuanced interpretation of semantic change, the relevance of Graded Change Detection within the broader context of historical linguistics becomes questionable.


\section{Related work}
%

\subsection{Graded Change Detection}

\subsection{Classification framework}

\section{Methodology}

To ensure a rigorous and systematic comparison among state-of-the-art (SOTA) approaches, we carefully selected four widely adopted and powerful form-based and sense-based methods. Each approach underwent evaluation under diverse conditions, as outlined in the classification framework proposed by Montanelli and Periti. These conditions included variations in languages, benchmarks, and embeddings derived from distinct models and layers.

For the sake of simplicity, we chose to assess the performance of different approaches using pre-trained models, aligning with the unsupervised nature of SemEval.

\subsection{Benchmarks}

Our comparative analysis leveraged all available benchmarks for the Graded Change Detection task, spanning various languages, time periods, and test set sizes. These benchmarks adhere to the novel annotation paradigm for word senses known as Word Usage Graphs (WUGs) (Schlechtweg et al., 2020, 2021b).

In this paradigm, human annotators provide semantic proximity judgments for pairs of word usages (Word-in-Context). These judgments are then encapsulated in a weighted graph and subjected to clustering via a graph clustering algorithm, as illustrated in Figure 1. Word sense clusters are consequently inferred from simple pairwise word usage judgments, obviating the need for explicit word sense definitions. The ground truth for lexical semantic change, represented as a continuous score of change, is computed for each target word by comparing the cluster distributions of time-specific usages.

Details for each benchmark, including the current state-of-the-art performance for reference purposes, are presented in Table 1. A set of available benchmarks contains both the derived graded scores per target word and the raw judgments provided by annotators for every annotated pair. To ensure the most controlled experiment, we decided to compare approaches in detecting changes in the sentences used for building the graph instead of using the full corpora from which sentences were extracted. This means that our corpora C1 and C2 are represented by all and only the sentences from C1 and from C2 annotated.

\subsection{Contextualized Word Embeddings}

In our comparison, we included the most commonly used contextualized models, both monolingual and multilingual, such as BERT, mBERT, and XLM-R for each benchmark. Additionally, we incorporated a novel model that has recently achieved state-of-the-art performance in English, Swedish, Latin, and [mention the additional language]. Our pipeline is consistent for every model. Given a word, we collect contextualized word embeddings by individually feeding the models with each sentence in which the word occurs (i.e., word usage). We then extract contextualized embeddings generated at the top (i.e., last layer) of the model for the word in the input context. We rely on the contextualized nature of these representations for detecting and ranking signals of meaning change.

\subsection{Measuring Semantic Change}
APD
PRT
AP
WiDiD

\subsection{Experimental results}
\subsection{Form-based vs Sense-based}
\subsection{Time-oblivious vs Time-aware}



\begin{table*}[!ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccc}
 &  &  & \textbf{EN} & \textbf{LA} & \textbf{DE} & \textbf{SV} & \textbf{ES} & \multicolumn{3}{c}{\textbf{RU}} & \multicolumn{2}{c}{\textbf{NO}} & \textbf{ZH} \\ \cline{4-14} 
 &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textit{$C_1 - C_2$}} & \multicolumn{1}{c|}{\textit{$C_1 - C_2$}} & \multicolumn{1}{c|}{\textit{$C_1 - C_2$}} & \multicolumn{1}{c|}{\textit{$C_1 - C_2$}} & \multicolumn{1}{c|}{\textit{$C_1 - C_2$}} & \textit{$C_1 - C_2$} & \textit{$C_2 - C_3$} & \multicolumn{1}{c|}{\textit{$C_1 - C_3$}} & \textit{$C_1 - C_2$} & \multicolumn{1}{c|}{\textit{$C_2 - C_3$}} & \multicolumn{1}{c|}{\textit{$C_1 - C_2$}} \\ \cline{2-14} 
\multicolumn{1}{l|}{\multirow{2}{*}{\rotatebox{90}{\textbf{form-based}}}} & \multicolumn{1}{c|}{APD} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BERT\\ mBERT\\ XLM-R\\ XLL\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.563\\ .363\\ .444\\ \textbf{.886}*\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-\\ .102\\ .151\\ \textbf{.231}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.271\\ .398\\ .264\\ \textbf{.839}*\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.270\\ .389\\ .257\\ \textbf{.812}*\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.336\\ .401\\ .342\\ \textbf{.560}*\end{tabular}} & \begin{tabular}[c]{@{}c@{}}.518\\ .368\\ .290\\ \textbf{.796}*\end{tabular} & \begin{tabular}[c]{@{}c@{}}.482\\ .345\\ .287\\ \textbf{.820}*\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.416\\ .386\\ .318\\ \textbf{.863}*\end{tabular}} & \begin{tabular}[c]{@{}c@{}}.441\\ .279\\ .195\\ \textbf{.659}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.466\\ .488\\ .379\\ \textbf{.640}*\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.656\\ .689\\ .500\\ \textbf{.731}*\end{tabular}} \\ \cline{2-14} 
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{PRT} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BERT\\ mBERT\\ XLM-R\\ XLL\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.457\\ .270\\ .411\\ \textbf{.676}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-\\ .380\\ .424\\ \textbf{.506}*\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.422\\ .436\\ .369\\ \textbf{.824}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.158\\ .193\\ .020\\ \textbf{.696}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.392\\ \textbf{.539}\\ .453\\ .494\end{tabular}} & \begin{tabular}[c]{@{}c@{}}.400\\ .391\\ .321\\ \textbf{.704}\end{tabular} & \begin{tabular}[c]{@{}c@{}}.374\\ .356\\ .443\\ \textbf{.750}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.347\\ .423\\ .405\\ \textbf{.727}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}.507\\ .219\\ .387\\ \textbf{.764}*\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.444\\ .438\\ .149\\ \textbf{.519}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{.712}\\ .524\\ .558\\ .699\end{tabular}} \\ \cline{2-14} 
\multicolumn{1}{l|}{\multirow{2}{*}{\rotatebox{90}{\textbf{sense-based}}}} & \multicolumn{1}{c|}{AP} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BERT\\ mBERT\\ XLM-R\\ XLL\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.289\\ .181\\ .278\\ \textbf{.493}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-\\ .277\\ \textbf{.398}\\ .033\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.469\\ .280\\ .224\\ \textbf{.499}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}- .090\\ .023\\  -.076\\ \textbf{.118}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.210\\ .101\\ .126\\ \textbf{.278}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}.069\\ .017\\ - .068\\ \textbf{.106}\end{tabular} & \begin{tabular}[c]{@{}c@{}}.279\\ .086\\ \textbf{.209}\\ .053\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.094\\ - .116\\ \textbf{.130}\\ .117\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\textbf{.314}\\ .035\\ - .100\\ .297\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.011\\ - .090\\ .030\\ \textbf{.381}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.165\\ .465\\ .448\\ \textbf{.308}\end{tabular}} \\ \cline{2-14} 
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{WiDiD} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BERT\\ mBERT\\ XLM-R\\ XLL\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.385\\ .323\\ .564\\ \textbf{.652}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}-\\ - .0.39\\ - .064\\ \textbf{.236}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.355\\ .312\\ .499\\ \textbf{.677}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.106\\ .195\\ .129\\ \textbf{.475}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.251\\ .417\\ .390\\ \textbf{.417}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}.135\\ - .068\\ \textbf{.268}\\ .178\end{tabular} & \begin{tabular}[c]{@{}c@{}}.102\\ .160\\ .216\\ \textbf{.354}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.243\\ .142\\ .342\\ \textbf{.364}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}.233\\ .241\\ .226\\ \textbf{.561}\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.087\\ .290\\ .349\\ \textbf{.457}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}.533\\ .338\\ .382\\ \textbf{.563}\end{tabular}} \\ \cline{2-14} 
\end{tabular}%
}
\caption{Todo}
\label{tab:form-vs-sense}
\end{table*}
\cite{pilehvar2019wic}

%notes: è normale hce i modelli form siano più avantaggiati poichè mancano di uno step intermedio

Why? -> Word-in-Context
Word Sense Induction
Semantic Change

\subsection{Other dimension of comparison}
\paragraph{Layers}
\paragraph{Layers aggregation}
\paragraph{Monolingual vs Multilingual}
\paragraph{Semantic change measures}
Are models time-awarness? Can model contextualize?
are cosine best for LSC?
are the last four layers the best for addressing LSC?
are monolingual model better for addressing LSC?

\section{Time-aware vs. Time-oblivious: Should we model time-aware model?}
The consideration of time awareness in embedding models focuses on how temporal information is integrated into the model when processing documents. Time-oblivious approaches operate under the assumption that a document at time t inherently adopts linguistic patterns reflective of the language at the same time, rendering unnecessary the explicit incorporation of time information into the embedding model. In contrast, time-aware approaches assume that contextualized embedding models face challenges in adapting to temporal shifts and generalizing over time, as they are typically pre-trained on corpora derived from a snapshot of the web collected at a specific moment. Given that our model demonstrates transfer learning capabilities across languages, we posit that the model can adapt to temporal changes within the same languages as most of significant portion of words maintains stability over time\cite{}. Despite the contextualization potential of models, especially in cross-linguistic scenarios, caution is warranted when working with a small language unit, such as word occurrences. Even though contextualized models can adapt to linguistic changes, they fall short when it comes to contextualizing word meanings beyond their training scope. This limitation is demonstrated through simple experiments emulating semantic change, detailed in our forthcoming paper X [currently under review].

This limitation underscores the advantages of form-based approaches in Grand Change Detection. Given the model's inability to contextualize word meanings beyond their training data, clustering algorithms struggle to disambiguate meanings for which the model lacks training. In contrast, form-based approaches can leverage embeddings that are more spatially distant to effectively model semantic changes.



\section{Supervised vs Unsupervised: is supervision the way?}
Approaches leveraging a form of supervision have demonstrated significantly greater efficacy for Lexical Semantic Change (LSC) than unsupervised models. We posit that supervision should be embraced to enhance the contextualization capabilities of the model or its awareness of the underlying meaning it was trained upon, rather than merely augmenting its 'pre-trained' knowledge of word meanings. This is particularly crucial given the dynamic nature of language or few-resources languages; meanings that diverge from the injected pre-trained knowledge may be inadequately represented, echoing the challenges faced by unsupervised models of semantic change.

While it is undeniable that models like GPT showcase exceptional proficiency in generating sense definitions, representing the forefront of AI with continuous updates, their strength lies in modeling present and future definitions. However, they might falter when tasked with producing definitions for the past, as exemplified in Table X. Therefore, we contend that fine-tuning may offer a more adaptable approach, even in the absence of explicit supervision.



\section{XL-Lexeme vs ChatGPT per LSC}

\section{Towards a new generation LSC}
massive graded change ha senso solo over time petr torvare il punto di cambiamento
binary change is not reliable dobbiamo rimodellarlo
dobbiamo modellare binary e sense -> 


\section{Related work}

\section{Conclusion}

%However, since the GCD tasks is charachterized by small-size benchmarks~(e.g.,~31 target words,~\citealp{schlechtweg2020semeval}), different evaluation settings hinders a fair and consistent performance comparison. This is especially true as recent work has shown that semantic change estimates derived by contextualized embeddings are often inflated or underestimated~\cite{liu2021statistically}, and that statistical correlation with gold labels can be obtained by using random scores as a degree of change~\cite{zhou2023finer}.  
%, often characterized by a skewed distribution of change scores~\cite{kutuzov2020uio}\footnote{This means that human annotators assigned the same judgment to most instances},
%the evaluation and comparison of the approaches for GCD may be particularly prone to be biased. This is especially true as recent work has shown that semantic change estimates are often inflated or underestimated~\cite{liu2021statistically}, and that statistical correlation with gold labels can be obtained by using random scores as a degree of change~\cite{zhou2023finer}.
%As a result, current performance comparison are prone to be bias as they relied on benchmark characterized by limited test set~(e.g.,~31 target words,~\citealp{schlechtweg2020semeval}), often characterized by a skewed distribution of change scores~\cite{kutuzov2020uio}\footnote{This means that human annotators assigned the same judgment to most instances}

%Since most available benchmarks comprise a limited test set~(e.g.,~31 target words,~\citealp{schlechtweg2020semeval}), often characterized by a skewed distribution of change scores~\cite{kutuzov2020uio}\footnote{This means that human annotators assigned the same judgment to most instances}, the evaluation and comparison of the approaches for GCD may be particularly prone to be biased. This is especially true as recent work has shown that semantic change estimates are often inflated or underestimated~\cite{liu2021statistically}, and that statistical correlation with gold labels can be obtained by using random scores as a degree of change~\cite{zhou2023finer}.

%Moreover, current evaluations of contextualized models for GCD involves only a partial complexity inherent to the LSC problem.







